The Communication-Friendly Privacy-Preserving Machine Learning against Malicious Adversaries

With the increasing emphasis on privacy regulations, such as GDPR, protecting individual privacy and ensuring compliance have become critical concerns for both individuals and organizations. Privacy-preserving machine learning (PPML) is an innovative approach that allows for secure data analysis while safeguarding sensitive information. It enables organizations to extract valuable insights from data without compromising privacy. Secure multi-party computation (MPC) is a key tool in PPML, as it allows multiple parties to jointly compute functions without revealing their private inputs, making it essential in multi-server environments. We address the performance overhead of existing maliciously secure protocols, particularly in finite rings like $\mathbb{Z}_{2^\ell}$, by introducing an efficient protocol for secure linear function evaluation. We implement our maliciously secure MPC protocol on GPUs, significantly improving its efficiency and scalability. We extend the protocol to handle linear and non-linear layers, ensuring compatibility with a wide range of machine-learning models. Finally, we comprehensively evaluate machine learning models by integrating our protocol into the workflow, enabling secure and efficient inference across simple and complex models, such as convolutional neural networks (CNNs).

==> subject/buildingblock.tex <==
%!TEX root = ../main.tex
\section{Building block}

%1/讲本段内容
%2/讲postprocessing
\noindent In this section, we initially present our multiplication verification protocol designed for ring operation. Following that, we introduce our lookup table-based verification method specifically designed for verifying evaluation of nonlinear functions.


\subsection{Batch Multiplication verification}

%For any multi-fan-In polynomial evaluation result $\{\langle x_1 \rangle,\ldots,\langle x_n \rangle;\langle y \rangle\}$ of relationship $F^d(x_1,\ldots,x_n) = y$, we propose a verifivation protocol that is secure against a active, static adversary. 

%\noindent\textbf{Robustness of Reconstruction.} Our protocol is based on a 2-out-of-3 additively secret sharing scheme. It possesses the 1-robustness property of reconstruction. In other words, when it comes to a share $\langle \cdot \rangle$, a single corrupted party cannot deceive the honest parties into accepting an incorrect reconstruction result. This is because any two honest parties can collaborate to reconstruct the secret value and verify the correctness of the result.

 %A line of works \cite{nv18, GS20, ATLAS, Brain} apply batch multiplication verification on Shamir secret sharing sheme, which migrate verifying the correctness of multiplication multiplications to verifying polynomial multiplications using polynomial interpolation. We refine and apply this idea on our multiplication verification with 2-out-of-3 additively secret sharing form.



%For verification of $N$ pairs of multiplication result $\{\langle x_i \rangle,\langle y_i \rangle; \langle z_i \rangle\}_{i \in |N|}$, a straightforward idea is to verify a dot product of $\Delta = \sum^N_{i = 1} \langle r^i \cdot x_i \rangle \cdot \langle y_i \rangle -  \langle r_i \cdot z_i \rangle $ with random challenge $r$ and reveal $\Delta$ to check it equal to zero. But there are two problems. One is that the adversary knows the deviation error of the calculation result, and it can introduce the same deviation error when calculating $\Delta$ to ensure that $\Delta$ is 0. The other is that the adversary can introduce a specific error in $z_i$ to make $\Delta$ extremely high probability to pass verification, such as introducing $e=2^{\lambda-1}$ to make $r^i \cdot (z_i+e) =z_i$ with a probability of 1/2.


\noindent To verify $N$ pairs of multiplication $\{\langle x_i \rangle, \langle y_i \rangle; \langle z_i \rangle\}_{i \in |N|}$, a straightforward approach is to transfer to verify that dot product $\Delta = \sum^N_{i = 1} \langle r^i \cdot x_i \rangle \cdot \langle y_i \rangle - \langle r^i \cdot z_i \rangle$ equal to zero with the random challenge $r$. However, there are two issues with this approach.
The first problem is that the adversary is aware of the deviation error in the calculation results, allowing them to introduce the same deviation error when computing $\Delta$ to fabricate $\Delta=0$.
The second problem arises from the calculation within the ring, where the adversary can intentionally introduce a specific error in $z_i$, leading to a high probability of $\Delta$ passing the verification. For instance, the adversary can introduce an error $e = 2^{\lambda-1}$ in such a way that the equation $r^i \cdot (z_i+e) = r^i \cdot z_i$ holds with a probability of 1/2 for the even $r^i$.

To address the former problem, we introduce a random multiplication term. Our protocol make the parties turn to evaluate $\Delta = \langle \alpha \rangle \cdot (\sum^N_{i = 1} \langle r^i \cdot x_i \rangle \cdot \langle y_i \rangle - \langle r^i \cdot z_i \rangle)$ (using $\Pple$) with random share $\langle \alpha \rangle$. The adversary can only guess the value of $\alpha$ to pass verification with the probability $2^{-\lambda}$.
To tackle the latter problem, our approach is to locally transfer the shares into the polynomial ring $\ZZ_{2^\lambda}[x]/f(x)$, where $f(x)$ is a monomial of degree $\kappa$. By performing the verification in $\ZZ_{2^\lambda}[x]/f(x)$ instead of the original ring, the error introduced by the adversary can only pass the verification only if it is eliminated on every term of the polynomial ring, which reduces the probability to $2^{-\kappa}$.
Following this idea, we construct our batch multiplication verification protocol as follows.

\myhalfbox{ Protocol $\Ptran (\{\langle x_i \rangle,\langle y_i \rangle, \langle z_i \rangle\}_{i \in |N|})$}{white!40}{white!10}{
    \footnotesize

    \emph{Input:}  $N$ pairs of $\langle \cdot \rangle$-shared multiplication. 
    
    \emph{Output:} One pair of $N$-dimension $\langle \cdot \rangle^{\lambda[x]}$-shared dot product. 
    
    \underline{\textbf{Preprocessing:}}
    \begin{itemize}[leftmargin=*]
    	\item[-] All parties invoke $\langle r \rangle^{\lambda[x]}  \leftarrow \Pshc^{\lambda[x]}$ locally;
	
	
	\end{itemize}

    \smallskip
    
    \underline{\textbf{Online:}}
    \begin{itemize}[leftmargin=*]
    \item[-] All parties reconstruct $r$ with $\Prec$ and calculate $r^i$ for all ${i \in |N|}$.
    \item[-] All parties transfer $\langle \cdot \rangle$ to $\langle \cdot \rangle^{\lambda[x]}$ locally by setting the constant term of $\langle \cdot \rangle^{\lambda[x]}$ to $\langle \cdot \rangle$.
    \item[-] All parties set $\langle z \rangle^{\lambda[x]} := \sum^N_{i = 1} r^i \cdot \langle z_i \rangle^{\lambda[x]}$, and $\langle x'_i \rangle^{\lambda[x]} := r^i \cdot \langle x_i \rangle^{\lambda[x]}$ for all $i \in |N|$.
    \item[-] Return $\{\langle x_i \rangle^{\lambda[x]},\langle y_i \rangle^{\lambda[x]}\}_{i \in |N|}; \langle z \rangle^{\lambda[x]}$
    %\item[-] $P_0$ returns $([r_z]_1,[r_z]_2)$ and $P_j$, for $j \in \{1,2\}$, returns $([r_z]_j, m_z)$.
    \end{itemize}
         \medskip
    }{ The Dot Product Transformation   \label{fig:MTP}}

    
\noindent \textbf{Conversion to Dot Product.}
To verify the multiplication triples $\{\langle x_i \rangle, \langle y_i \rangle; \langle z_i \rangle\}_{i \in |N|}$, we first transfer them to the polynomial ring $\{\langle x_i \rangle^{\lambda[x]}, \langle y_i \rangle^{\lambda[x]}; \langle z_i \rangle^{\lambda[x]}\}_{i \in |N|}$. In this transformation, the constant coefficient of each target share is set to the original ring element and other's to $0$ (i.e.,$[r_{z_i}]^{\lambda[x]}_1 = \{[r_{z_i}]_1,0,\ldots,0\}$). Then, all parties invokes $\langle r \rangle^{\lambda[x]} \leftarrow \Pshc^{\lambda[x]}$ to generate a random value $r$ and reconstruct it with $\Prec$. All parties calculate $\langle z \rangle^{\lambda[x]} = \sum^N_{i = 1} r^i \cdot \langle z_i \rangle^{\lambda[x]}$, and $\langle x'_i \rangle^{\lambda[x]} = r^i \cdot \langle x_i \rangle^{\lambda[x]}$ for all $i \in |N|$ . At this point, all parties only need to verify that $\langle z \rangle^{\lambda[x]}  = \sum^N_{i = 1} \langle x'_i \rangle^{\lambda[x]} \cdot \langle y_i \rangle^{\lambda[x]}$. Note that if there exists any pair such that $x_i \cdot y_i \neq z_i$, the probability of equation holds is $2^{-\kappa}$. $\Ptran$(Fig.~\ref{fig:MTP}) outlines the transfering procedure. We prove the security of $\Ptran$ as follows.

\begin{lemma}
\label{transl}
The protocol $\Ptran$ securely transfers $N$ pairs of multiplication triples to a dot product pair with $2^{-\kappa}$ soundness error, in the presence of one malicious adversary.
\end{lemma}
\begin{proofsketch} It is sufficient to show that $r$ is uniform random if $\Prec$ is not abort. The adversary tries to make $z=\sum^N_{i = 1} r^i \cdot x_i \cdot y_i$ where $z_i = x_i \cdot y_i + e_i$ for $i \in |N|$ with an error list $\{e_i\}_{i \in |N|}$.
Expend $z$ to get $\sum^N_{i = 1} r^i \cdot x_i \cdot y_i = \sum^N_{i = 1} r^i\cdot( x_i \cdot y_i + e_i)$, the adversary's target is to forge $\sum^N_{i = 1} r^i \cdot e_i = 0$. Obviously, for the $\kappa$ degree polynomial ring element $r \in \ZZ_{2^\lambda}[x]$, the probability that the adversary deliberately chooses $e_i$ to make the equation hold is $2^{-\kappa}$.
 \end{proofsketch} 
%Since the cross-terms $r_\alpha \cdot r_{x_i}$, $r_\alpha \cdot r_{y_i}$, $r_{x_i} \cdot r_{y_i}$ need to be sent, this verification protocol requires an additional $3 \cdot \lambda \cdot N$ communication in the offline phase.

\myhalfbox{ Protocol $\Prd (\{\langle x_i \rangle^{\lambda[x]},\langle y_i \rangle^{\lambda[x]}\}_{i \in |N|};\langle z \rangle^{\lambda[x]})$}{white!20}{white!10}{
    \footnotesize
    
   	\emph{Input:}  $N$-dimension $\langle \cdot \rangle^{\lambda[x]}$-shared dot product. 
    
    \emph{Output:} $N/2$-dimension $\langle \cdot \rangle^{\lambda[x]}$-shared dot product. 
	
\underline{\textbf{Execution:}}
    \begin{itemize}[leftmargin=*]
    \item[-] For $i \in |N/2|$ and $j \in |n|$, all parties set
    \begin{itemize}
    \item  $\langle f_i(0) \rangle^{\lambda[x]} = \langle x_{2\cdot i - 1} \rangle^{\lambda[x]}$;$\langle f_i(1)\rangle^{\lambda[x]} = \langle x_{2\cdot i } \rangle$; $\langle f_i(2)\rangle^{\lambda[x]} =  2 \cdot\langle f_i(1) \rangle^{\lambda[x]} - \langle f_i(0) \rangle^{\lambda[x]}$.
    \item  $\langle g_i(0) \rangle^{\lambda[x]} = \langle x_{2\cdot i - 1} \rangle^{\lambda[x]}$;$\langle g_i(1)\rangle^{\lambda[x]} = \langle x_{2\cdot i } \rangle^{\lambda[x]}$; $\langle g_i(2)\rangle^{\lambda[x]} =  2 \cdot\langle g_i(1) \rangle^{\lambda[x]} - \langle g_i(0) \rangle^{\lambda[x]}$.
    \item  $\langle h(0) \rangle^{\lambda[x]} = \sum \langle f_i(0) \rangle^{\lambda[x]} \cdot \langle g_i(0) \rangle^{\lambda[x]}$;$\langle h(1)\rangle^{\lambda[x]} = \langle z \rangle^{\lambda[x]} - \langle h(0) \rangle^{\lambda[x]}$; $\langle h(2)\rangle^{\lambda[x]} = \sum \langle f_i(2) \rangle^{\lambda[x]} \cdot \langle g_i(2) \rangle^{\lambda[x]}$; 
    %\item For $k \in |d-1|$, $\langle h_j(k)\rangle =  \sum F^d(\langle f_1^i(k) \rangle, \ldots, \langle f_n^i(k) \rangle)$.
    \end{itemize}
    	\item[-] All parties invoke $\langle \delta \rangle^{\lambda[x]} \leftarrow \Pshc^{\lambda[x]}$ and reveal $\langle 2 \cdot \delta \rangle^{\lambda[x]}$. 
	\item[-] All parties calculate 
	\begin{itemize}
	\item $\langle h(\delta)\rangle^{\lambda[x]} =  \sum^{2}_{i = 0}((\Pi^{2}_{j=1,j\neq i}\frac{\delta-j}{i-j})\cdot \langle h(i)\rangle^{\lambda[x]})$.
	\item $\langle f_i(\delta)\rangle^{\lambda[x]} =  \delta \cdot\langle f_i(1) \rangle^{\lambda[x]} - (\delta - 1)\langle f_i(0) \rangle^{\lambda[x]}$.
	\item $\langle g_i(\delta)\rangle^{\lambda[x]} =  \delta \cdot\langle g_i(1) \rangle^{\lambda[x]} - (\delta - 1)\langle g_i(0) \rangle^{\lambda[x]}$.

	\end{itemize}
	\item[-] Return  $\{\langle f_{i}(\delta) \rangle^{\lambda[x]}, \langle g_{i}(\delta) \rangle^{\lambda[x]}\}_{i \in |N/2|}; \langle h(\delta)\rangle^{\lambda[x]}$.
    \end{itemize}

    \smallskip
}{ The Dot Product Dimension Reduce Protocol \label{fig:Reduce}} 




\noindent \textbf{Dimension reduction.}
We apply the technique of \cite{GS20} to reduce the demension of dot product $\langle z \rangle^{\lambda[x]}  = \sum^N_{i = 1} \langle x_i \rangle^{\lambda[x]} \cdot \langle y_i \rangle^{\lambda[x]}$. The reduce protocol $\Prd$  is shown in Fig.~\ref{fig:Reduce}. The idea of the $\Prd$ is to reduce verifying two multiplications at point $0,1$ to verifying one multiplication at point $\delta$ by linear interpolation. All parties do the following:
%We mainly introduce our multi-fan-in polynomial verification protocol in Fig.~\ref{fig:PPEV}. For $N$ pairs of polynomial evaluation result $\{\langle x^i_1 \rangle,\ldots,\langle x^i_n \rangle; \langle y^i \rangle\}_{i \in |N|}$, all parties process as following:
\begin{itemize}
\item Utilize $\langle x_{2i}\rangle^{\lambda[x]}$ and $\langle x_{2i-1}\rangle^{\lambda[x]}$ to interpolate a linear function, resulting in $N/2$ straight lines $\langle f_i(\cdot) \rangle^{\lambda[x]}$. Similarly, interpolate $\langle g_i(\cdot) \rangle^{\lambda[x]}$ with $\langle y_{2i} \rangle^{\lambda[x]}, \langle y_{2i-1} \rangle^{\lambda[x]}$.
\item  Calculate $\langle h(0) \rangle^{\lambda[x]} = \sum_{i=1}^{N/2} \langle f_i(0) \rangle^{\lambda[x]} \cdot \langle g_i(0) \rangle^{\lambda[x]}$ and $\langle h(2) \rangle^{\lambda[x]}= \sum_{i=1}^{N/2} \langle f_i(2)\rangle^{\lambda[x]} \cdot \langle g_i(2)\rangle^{\lambda[x]}$ with $\Pple^{\lambda[x]}$.
\item Calculate $\langle h(1) \rangle^{\lambda[x]}= \langle z \rangle^{\lambda[x]} - \langle h(0)\rangle^{\lambda[x]} $ and interpolate the dot product function  $\langle h(\cdot) \rangle^{\lambda[x]}$ with $\langle h(0) \rangle^{\lambda[x]},\langle h(1) \rangle^{\lambda[x]},\langle h(2) \rangle^{\lambda[x]}$.
\item Generate the random challenge $\delta \in \ZZ_{2^\lambda}[x]/f(x)$ through $\Pshc^{\lambda[x]}$;  To ensure that the interpolation is divisible, let $\delta = \delta \cdot 2$.
\item Calculate $\langle h(\delta) \rangle^{\lambda[x]}, \langle f_i(\delta) \rangle^{\lambda[x]}$ locally with the interpolated function $\langle h(\cdot) \rangle^{\lambda[x]},\langle f_i(\cdot) \rangle^{\lambda[x]}$; 
\item Return new list $\{\langle f_i(\delta) \rangle^{\lambda[x]}\}_{i \in |N/2|}$, $\langle h(\delta)\rangle^{\lambda[x]}$.
\end{itemize}
%The security of verification protocol is based on: the adversary can not predict $\delta$ so that the adversary cannot introduce correct error on $\langle h(0) \rangle$ and $\langle h(2) \rangle$ to make $\langle h(\delta) \rangle = \sum_{i=1}^{N/2}   \langle f_i(\delta)\rangle \cdot \langle g_i(\delta)\rangle$.
Note that points $0$, $1$, $2$ refer to monomials with constant coefficient of $0$, $1$, and $2$ in $\ZZ_{2^\lambda}[x]/f(x)$.
Each call of $\Prd$ can reduce the dot product dimension that needs to be verified to one-half. The additional overhead required for each call is one round and communication of $8 \lambda\cdot \kappa$ bits in the online phase and communication of $\lambda\cdot \kappa$ bits in the offline phase. 
We perform $R$ times $\Prd$ to reduce the dot product to dimension $N / \log R$, which remains the part $\sum^{N / \log R}_{i = 1}\langle f_i(\delta) \rangle^{\lambda[x]} \cdot \langle g_i(\delta) \rangle^{\lambda[x]}=\langle h(\delta) \rangle^{\lambda[x]}$ to be verified. We prove the security of $\Prd$ as follows.
%During the dimension reduction step, the final verified equation $\langle f(\delta) \rangle^{\lambda[x]} \cdot \langle g(\delta) \rangle^{\lambda[x]}=\langle h(\delta) \rangle^{\lambda[x]}$ is obtained by invoking $\Prd$ a total of $\log N$ times.
%Our multiplication protocol $\Pmulv$ (Fig.~\ref{fig:PPEV}) first transfer $N$ pairs of multiplication verification into dot product verification with $N$-dimension. Then $\Pmulv$ invoke $R$ times to get a $N/2^R$-dimension dot product to verify and utilize $\Pvdot$ to verify the correctness of it with $3\lambda N/2^R$ extra communication in the setup phase and $2 \cdot \lambda$ in the online phase.

\begin{lemma}
\label{polyred}
The protocol $\Prd$ securely transfers a $N$-dimension dot product to a $N/2$-dimension dot product pair with $2^{-\kappa}$ soundness error, in the presence of one malicious adversary.
\end{lemma}
 \begin{proofsketch} For the convenience of description, we denote $h'(k)=\sum^{N/2}_{i = 1} f_i(k) \cdot g_i(k)$. The adversary tries to make $h(\delta) = h'(\delta)$ when $h(0) + h(1) = h'(0) + h'(1) + e$ (we denote $e$ the error introduced in $z$). At the same time, the adversary can introduce new errors $e_1, e_2$ when calculating $h(0)$ and $h(2)$ so that $h(0) = h'(0) + e_1, h(1) = h'(1) + e - e_1, h(2) = h'(2) + e_2$. 
 Considering 
 $ h(\delta)=  \sum^{2}_{i = 0}((\Pi^{2}_{j=1,j\neq i}\frac{\delta-j}{i-j})\cdot  h(i)) = \frac{(\delta - 1)\cdot(\delta - 2)}{2} \cdot h(0) + \delta \cdot (2 - \delta) \cdot h(1) + \frac{(\delta - 1)*\delta}{2} \cdot h(2)$, to make it equal to $h'(\delta) = \frac{(\delta - 1)\cdot(\delta - 2)}{2} \cdot h'(0) + \delta \cdot (2 - \delta) \cdot h'(1) + \frac{(\delta - 1)*\delta}{2} \cdot h'(2)$, is to make $\frac{(\delta - 1)\cdot(\delta - 2)}{2} \cdot e_1 + \delta \cdot (2 - \delta) \cdot (e - e_1) + \frac{(\delta - 1)*\delta}{2} \cdot (e_2) = 0$ for random picked $\delta \in \ZZ_{2^\lambda}[x]$. The probability that the adversary deliberately chooses $e, e_1, e_2$ to make the equation holds is $2^{-\kappa}$.
 \end{proofsketch} 

\myhalfbox{ Protocol $\Pvdot (\{\langle x_i \rangle^{\lambda[x]},\langle y_i \rangle^{\lambda[x]}\}_{i\in |N|}; \langle z \rangle^{\lambda[x]})$}{white!20}{white!10}{
    \footnotesize
   	\emph{Input:}  A $N$-dimension $\langle \cdot \rangle^{\lambda[x]}$-shared dot product pair. 
    
    \emph{Output:}  $z \overset{?}{=} \sum^N_{i = 1} x_i \cdot y_i$. 

\underline{\textbf{Execution:}}
    \begin{itemize}[leftmargin=*]
    \item[-] All parties invoke $\langle \alpha \rangle^{\lambda[x]} \leftarrow \Pshc^{\lambda[x]}$.
    \item[-] All parties calculate $\langle \Delta \rangle^{\lambda[x]}  = \langle \alpha \rangle^{\lambda[x]} \cdot (\sum^N_{i = 1}\langle x_i \rangle^{\lambda[x]} \cdot \langle y_i \rangle^{\lambda[x]} - \langle z \rangle^{\lambda[x]})$ with $\Pple^{\lambda[x]}$.
    \item[-] All parties call $\Delta = \Prec^{\lambda[x]}(\langle \Delta \rangle^{\lambda[x]})$.
    \item[-] return $1$ if $\Delta = 0$, otherwise $0$.
    	    \end{itemize}

    \smallskip
}{ The Dot Product Verification Protocol \label{fig:DPV}} 


\noindent \textbf{Dot Product Verification.}
As mentioned previously, we can incorporate a random multiplication term to validate a dot product triple. For verification of $\sum^{N / \log R}_{i = 1}\langle f_i(\delta) \rangle^{\lambda[x]} \cdot \langle g_i(\delta) \rangle^{\lambda[x]}=\langle h(\delta) \rangle^{\lambda[x]}$, $\Pvdot$ (Fig.~\ref{fig:DPV}) turns to verify $\langle \alpha \rangle^{\lambda[x]} \cdot (\sum^{N / \log R}_{i = 1}\cdot \langle x_i \rangle^{\lambda[x]} \cdot \langle y_i \rangle^{\lambda[x]} - \langle  z_i \rangle^{\lambda[x]})$ equal to zero. We prove the security of $\Pvdot$ as follows.

\begin{lemma}
\label{polyvv}
The protocol $\Pvdot$ securely verifies a $N$-dimension dot product with $2^{-\kappa}$ soundness error, in the presence of one malicious adversary.
\end{lemma}
%Since the $\Pvdot$ reconstructs a non-random number $\Delta$, privacy needs to be investigated.
\begin{proofsketch} 
 
 \textbf{Soundness}: It is trivial to show that $\alpha$ is uniformly random and unknown to the adversary. Therefore, for $z = \sum^N_{i = 1}  x_i \cdot y_i + e$, we have $\Delta = \alpha \cdot e + e_1$ where $e_1$ is introduced when evaluating $\Pple$. Due to $e_1$ is independent of $\alpha$ via Claim.~\ref{polyevall}, the probability that the adversary deliberately chooses $e, e_1$ to make $\Delta = 0$ is $2^{-\kappa}$.
\textbf{Privacy}: Since $\alpha$ is completely random, the adversary get no information about $e$
 \end{proofsketch} 
%As mentioned before, we can introduce a random multiplication term to verify a dot product triple. To verify $\sum^{N / \log R}_{i = 1}\langle f_i(\delta) \rangle^{\lambda[x]} \cdot \langle g_i(\delta) \rangle^{\lambda[x]}=\langle h(\delta) \rangle^{\lambda[x]}$, all parties reveal $\Delta = \langle \alpha \rangle^{\lambda[x]} \cdot \langle x_i \rangle^{\lambda[x]} \cdot \langle y_i \rangle^{\lambda[x]} - \langle \alpha \rangle^{\lambda[x]} \langle  z_i \rangle^{\lambda[x]}$ and check it equal to zero in $\ZZ_{2^\lambda}[x]/f(x)$.

\myhalfbox{ Protocol $\Pmulv (\{\langle x_i \rangle,\langle y_i \rangle; \langle z_i \rangle\}_{i \in |N|}, R)$}{white!20}{white!10}{
    \footnotesize
    \emph{Input:}  $N$ pairs of $\langle \cdot \rangle$-shared multiplication. 
    
    \emph{Output:}  $z_i \overset{?}{=}  x_i \cdot y_i$ for all $i \in |N|$. 
    
   \underline{\textbf{Execution:}}	
    \begin{itemize}[leftmargin=*]
    \item[-] All parties invoke $\Ptran(\{\langle x_i \rangle,\langle y_i \rangle; \langle z_i \rangle\}_{i \in |N|})$ to get $\{\langle x_i \rangle^{\lambda[x]},\langle y_i \rangle^{\lambda[x]}\}_{i \in |N|};\langle z \rangle^{\lambda[x]}$.
    \item[-] For $k = 1,\ldots, R$, all parties perform:
       \begin{itemize}
   	\item $\{\{\langle x_i \rangle^{\lambda[x]},\langle y_i \rangle^{\lambda[x]}\}_{i \in |N/2^{k}|};\langle z \rangle^{\lambda[x]} \} \leftarrow \Prd (\{\langle x_i \rangle^{\lambda[x]},\langle y_i \rangle^{\lambda[x]}\}_{i \in |N/2^{k - 1}|};\langle z \rangle^{\lambda[x]})$
	\end{itemize}
	\item[-] All parties call $\Delta = \Pvdot (\{\langle x_i \rangle^{\lambda[x]},\langle y_i \rangle^{\lambda[x]}\}_{i \in |N/2^R|};\langle z \rangle^{\lambda[x]})$
	\item[-] Return $\Delta$.
    \end{itemize}

    \smallskip
}{ The Batch Multiplication Verification Protocol \label{fig:PPEV}} 


Our batch multiplication verification protocol $\Pmulv$ in Fig.~\ref{fig:PPEV} integrates the above three phases, which requires $1$ rounds and communication of $(R + 3N/2^R + 1)\lambda \cdot \kappa $ bits in the offline phase and requires $R+2$ rounds and communication of $(10R + 8)\lambda \cdot \kappa $ bits in the online phase for $N$ pairs of multiplication triples. The security proof of $\Pmulv$ is as follows.  

\begin{theorem}
\label{multvv}
The protocol $\Pmulv$ securely verifies $N$ pairs of multiplication triples with $2^{R +2 - \kappa}$ soundness error, in the presence of one malicious party.
\end{theorem}
\begin{proofsketch} 
 
 \textbf{Soundness}: From Lemma.~\ref{transl}, Lemma.~\ref{polyred} and Lemma.~\ref{polyvv}, we know that the adversary has $R+2$ chances with probability $2^{-\kappa}$ to pass the verification.
Therefore the probability that the adversary success is $1 - (1 - 2^{-\kappa})^{R+2} \approx 2^{R+2-\kappa}$.
\textbf{Privacy}: From Lemma.~\ref{polyvv}, the adversary get no information about $e$ of $\Prd$ outpus. Therefore, the adversary cannot break privacy by introducing input-related information in $e$.
 \end{proofsketch} 
%\textbf{Security up to additively attack.} 
%If $\Delta \neq 0$, the adversary gains information about the error introduced at a specific point, which impacts the value of the polynomial $h(\cdot)$ at the $\delta$ point.  Since the degree of $h(\cdot)$ is greater than or equal to two, such information obtained by the adversary does not reveal any intelligence about the coefficients.





 %\myhalfbox{ Protocol $\Pplv (\{\langle x^i_1 \rangle,\ldots,\langle x^i_n \rangle; \langle y^i \rangle\}_{i \in |N|})$}{white!20}{white!10}{
%    \footnotesize
%   	
%    \begin{itemize}[leftmargin=*]
%    \item[-] All parties agree upon a seed and generate random list $\{r_1,\ldots, r_{N/2}\}$.
%    \item[-] All parties set $n\cdot N/2$ linear function $\langle f_j^i(k) \rangle= (\langle x_j^{2i}\rangle - \langle x_j^{2i-1}\rangle) k + \langle x_j^{2i-1}\rangle$ for each $i\in|N/2|, j\in|n|$.
%    	\item[-] For $k \in |2, d+1|$, all parties calculate $\langle h'(k)\rangle  = \sum_{i=1}^{N/2} r_i \cdot F^d( f_1^i(k) \rangle, \ldots, \langle f_n^i(k) \rangle) $. 
%	\item[-] All parties calculate $\langle h'(0)\rangle = \sum_{i=1}^{N/2} r_i \cdot  \langle y^{2i - 1} \rangle$ and $\langle h'(1)\rangle= \sum_{i=1}^{N/2} r_i \cdot  \langle y^{2i} \rangle$. 
%	\item[-] All parties interpolate shared polynomials locally as $\langle h'(k) \rangle = \sum^{d}_{i = 0}((\Pi^{d}_{j=1,j\neq i}\frac{k-j}{i-j})\cdot \langle h'(i)\rangle)$ and $\langle \vec{g}(y) \rangle$ similarly.
%	\item[-] All parites pick a random coin $\delta>d-1$,  calculate $\langle h(\delta)\rangle  = \sum_{i=1}^{N/2} r_i \cdot F^d( f_1^i(\delta) \rangle, \ldots, \langle f_n^i(k) \rangle) $ and evaluate $\langle h'(\delta) \rangle$ locally with $\langle h(k) \rangle$.
%	\item[-] All parties reconstruct $\Delta = \langle h(\delta) \rangle - \langle h'(\delta) \rangle$, return $1$ if $\Delta = 0$, $0$ else. 
%    \end{itemize}
%
%    \smallskip
%}{ The Batch-size Multi-Fan-In Polynomial Verification Protocol \label{fig:PPEV}} 



%\begin{lemma}
%\label{polyverifycomm}
%
%Protocol $\Pmulv$ for $N$ pairs of multiplication triple requires $R+2$ rounds and comunication of $2\cdot \lambda \cdot R + 2\cdot \lambda$ bits in the online phase and requires $1$ rounds and comunication of $\lambda \cdot R + 3\cdot \lambda \cdot N / 2^R$ bits in the online phase.
%\end{lemma}
 
% \begin{proof}
%Correctness: We use $h(i)$ to denote the polynomial calculated by $\langle f_j^i(k) \rangle$, and $h'(i)$ denote the interpolated polynomial from $h'(0) = h(0) + e_0, \ldots, h'(d) = h(d) + e_d$. For a random $\delta$, to pass the verification $\Delta = 0$, the adversary needs to introduce an error $\alpha e_\delta$ where $e_\delta$ is predicted from list $e_0,\ldots, e_d$, and $\alpha$ is a secret unknown to the adversary.
% \end{proof}   
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt  
\tikzset{global scale/.style={
    scale=#1,
    every node/.append style={scale=#1}
  }
}     
\begin{figure}%
  \centering
\begin{subfigure}[t]{.48\linewidth}
\parbox[][2cm][c]{\linewidth}{
  \centering
  \begin{tabular}{|c|c|}
\hline

$T(0)$                    & $\mathcal{C}(0,m_x)$                       \\ \hline
...                  &                                \\ \hline
$T(r)$                    & $\mathcal{C}(r,m_x)$                       \\ \hline

...                  &                                \\ \hline
$T(2^\ell-1)$ & $\mathcal{C}(2^\ell-1, m_x)$ \\ \hline
\end{tabular}
}
\caption{Look-up table $T$ with size $2^\ell$}
\end{subfigure}
\begin{subfigure}[t]{.48\linewidth}
\parbox[][2cm][c]{\linewidth}{
\centering
  \begin{tabular}{C}
% Don't indent the lstlisting environment!          
\\
  \mathcal{C}(r_x,m_x) := \\ \sum^{2^\ell}_j (j \overset{\text{?}}{=} r_x) \cdot T(j)
\\
\end{tabular}
}
  \caption{Look-up table Output}
 \end{subfigure}
 \caption{ Look-up table with variable $r$}%
  \label{fig:table}%
\end{figure}
 \begin{figure}[t]

\centering
  \begin{tabular}{C}
% Don't indent the lstlisting environment!          
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1,scale = 0.5, every node/.append style={scale=0.75}]
%uncomment if require: \path (0,378); %set diagram left start at 0, and has height of 378

%Shape: Square [id:dp503715782935556] 
\draw   (64,16) -- (114,16) -- (114,66) -- (64,66) -- cycle ;
%Shape: Square [id:dp4539237251615681] 
\draw   (114,16) -- (164,16) -- (164,66) -- (114,66) -- cycle ;
%Shape: Square [id:dp3537094623132443] 
\draw   (164,16) -- (214,16) -- (214,66) -- (164,66) -- cycle ;
%Shape: Square [id:dp10133292369086122] 
\draw   (214,16) -- (264,16) -- (264,66) -- (214,66) -- cycle ;
%Shape: Square [id:dp9348933821378842] 
\draw   (264,16) -- (314,16) -- (314,66) -- (264,66) -- cycle ;
%Shape: Square [id:dp645042818550977] 
\draw   (314,16) -- (364,16) -- (364,66) -- (314,66) -- cycle ;
%Shape: Square [id:dp760908234245624] 
\draw   (364,16) -- (414,16) -- (414,66) -- (364,66) -- cycle ;
%Shape: Square [id:dp0662919970935626] 
\draw   (414,16) -- (464,16) -- (464,66) -- (414,66) -- cycle ;
%Shape: Square [id:dp45149077417041106] 
\draw   (464,16) -- (514,16) -- (514,66) -- (464,66) -- cycle ;
%Shape: Square [id:dp30901138289562624] 
\draw   (514,16) -- (564,16) -- (564,66) -- (514,66) -- cycle ;
%Shape: Square [id:dp5966893283256769] 
\draw   (564,16) -- (614,16) -- (614,66) -- (564,66) -- cycle ;
%Shape: Square [id:dp6089799953565356] 
\draw   (132,86) -- (182,86) -- (182,136) -- (132,136) -- cycle ;
%Shape: Square [id:dp49925674395745323] 
\draw   (182,86) -- (232,86) -- (232,136) -- (182,136) -- cycle ;
%Shape: Square [id:dp6399657461381577] 
\draw   (232,86) -- (282,86) -- (282,136) -- (232,136) -- cycle ;
%Shape: Square [id:dp7377425589814409] 
\draw   (282,86) -- (332,86) -- (332,136) -- (282,136) -- cycle ;
%Shape: Square [id:dp8685222789130245] 
\draw   (332,86) -- (382,86) -- (382,136) -- (332,136) -- cycle ;
%Shape: Square [id:dp5097281394510816] 
\draw   (382,86) -- (432,86) -- (432,136) -- (382,136) -- cycle ;
%Shape: Square [id:dp5733657692824228] 
\draw   (432,86) -- (482,86) -- (482,136) -- (432,136) -- cycle ;
%Shape: Square [id:dp1592619804953751] 
\draw   (482,86) -- (532,86) -- (532,136) -- (482,136) -- cycle ;
%Shape: Square [id:dp2613244882320296] 
\draw   (532,86) -- (582,86) -- (582,136) -- (532,136) -- cycle ;
%Shape: Square [id:dp4301638749620038] 
\draw   (582,86) -- (632,86) -- (632,136) -- (582,136) -- cycle ;
%Shape: Square [id:dp8596933994035911] 
\draw   (632,86) -- (682,86) -- (682,136) -- (632,136) -- cycle ;
%Shape: Square [id:dp7376819933970904] 
\draw   (94,226) -- (144,226) -- (144,276) -- (94,276) -- cycle ;
%Shape: Square [id:dp6813134315100701] 
\draw   (144,226) -- (194,226) -- (194,276) -- (144,276) -- cycle ;
%Shape: Square [id:dp9810623203241053] 
\draw   (194,226) -- (244,226) -- (244,276) -- (194,276) -- cycle ;
%Shape: Square [id:dp6573322326794586] 
\draw   (244,226) -- (294,226) -- (294,276) -- (244,276) -- cycle ;
%Shape: Square [id:dp4099988342787533] 
\draw   (294,226) -- (344,226) -- (344,276) -- (294,276) -- cycle ;
%Shape: Square [id:dp2963187352493366] 
\draw   (344,226) -- (394,226) -- (394,276) -- (344,276) -- cycle ;
%Shape: Square [id:dp3836945306203391] 
\draw   (394,226) -- (444,226) -- (444,276) -- (394,276) -- cycle ;
%Shape: Square [id:dp49717567699211673] 
\draw   (444,226) -- (494,226) -- (494,276) -- (444,276) -- cycle ;
%Shape: Square [id:dp12515808417536267] 
\draw   (494,226) -- (544,226) -- (544,276) -- (494,276) -- cycle ;
%Shape: Square [id:dp7326739024726082] 
\draw   (544,226) -- (594,226) -- (594,276) -- (544,276) -- cycle ;
%Shape: Square [id:dp20807110333441137] 
\draw   (594,226) -- (644,226) -- (644,276) -- (594,276) -- cycle ;
%Curve Lines [id:da4247794852044885] 
\draw    (662,135.5) .. controls (650.24,149.22) and (646.16,151.42) .. (616.83,154.32) ;
\draw [shift={(615,154.5)}, rotate = 354.47] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp33087610467608397] 
\draw   (92,162.7) .. controls (92,158.45) and (95.45,155) .. (99.7,155) -- (635.3,155) .. controls (639.55,155) and (643,158.45) .. (643,162.7) -- (643,185.8) .. controls (643,190.05) and (639.55,193.5) .. (635.3,193.5) -- (99.7,193.5) .. controls (95.45,193.5) and (92,190.05) .. (92,185.8) -- cycle ;
%Curve Lines [id:da35120825871071215] 
\draw    (64,66) .. controls (60.02,105.8) and (64.95,141.14) .. (136.91,155.29) ;
\draw [shift={(138,155.5)}, rotate = 190.86] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7108612078863181] 
\draw    (91,66.5) -- (152.09,85.89) ;
\draw [shift={(154,86.5)}, rotate = 197.61] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7802963229087341] 
\draw    (139,65.5) -- (200.09,84.89) ;
\draw [shift={(202,85.5)}, rotate = 197.61] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da6300848027191612] 
\draw    (194,65.5) -- (255.09,84.89) ;
\draw [shift={(257,85.5)}, rotate = 197.61] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da5215783205459723] 
\draw    (246,65.5) -- (307.09,84.89) ;
\draw [shift={(309,85.5)}, rotate = 197.61] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da8425007497055648] 
\draw    (294,66.5) -- (355.09,85.89) ;
\draw [shift={(357,86.5)}, rotate = 197.61] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da42295666080935423] 
\draw    (344,66.5) -- (405.09,85.89) ;
\draw [shift={(407,86.5)}, rotate = 197.61] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7678591759761498] 
\draw    (392,66.5) -- (453.09,85.89) ;
\draw [shift={(455,86.5)}, rotate = 197.61] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da8734911913466622] 
\draw    (444,65.5) -- (505.09,84.89) ;
\draw [shift={(507,85.5)}, rotate = 197.61] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da14588803703271824] 
\draw    (492,66.5) -- (553.09,85.89) ;
\draw [shift={(555,86.5)}, rotate = 197.61] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da27433212657286843] 
\draw    (542,65.5) -- (603.09,84.89) ;
\draw [shift={(605,85.5)}, rotate = 197.61] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da9058653365193533] 
\draw    (595,66.5) -- (656.09,85.89) ;
\draw [shift={(658,86.5)}, rotate = 197.61] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da78942793141982] 
\draw    (365,195.5) -- (365,223.5) ;
\draw [shift={(365,225.5)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (83,33.4) node [anchor=north west][inner sep=0.75pt]    {$0$};
% Text Node
\draw (133,33.4) node [anchor=north west][inner sep=0.75pt]    {$0$};
% Text Node
\draw (433,33.4) node [anchor=north west][inner sep=0.75pt]    {$0$};
% Text Node
\draw (233,33.4) node [anchor=north west][inner sep=0.75pt]    {$0$};
% Text Node
\draw (333,33.4) node [anchor=north west][inner sep=0.75pt]    {$\delta $};
% Text Node
\draw (283,33.4) node [anchor=north west][inner sep=0.75pt]    {$0$};
% Text Node
\draw (183,33.4) node [anchor=north west][inner sep=0.75pt]    {$0$};
% Text Node
\draw (533,33.4) node [anchor=north west][inner sep=0.75pt]    {$0$};
% Text Node
\draw (583,33.4) node [anchor=north west][inner sep=0.75pt]    {$0$};
% Text Node
\draw (483,33.4) node [anchor=north west][inner sep=0.75pt]    {$0$};
% Text Node
\draw (383,33.4) node [anchor=north west][inner sep=0.75pt]    {$0$};
% Text Node
\draw (151,103.4) node [anchor=north west][inner sep=0.75pt]    {$0$};
% Text Node
\draw (201,103.4) node [anchor=north west][inner sep=0.75pt]    {$0$};
% Text Node
\draw (501,103.4) node [anchor=north west][inner sep=0.75pt]    {$0$};
% Text Node
\draw (301,103.4) node [anchor=north west][inner sep=0.75pt]    {$0$};
% Text Node
\draw (401,103.4) node [anchor=north west][inner sep=0.75pt]    {$0$};
% Text Node
\draw (351,103.4) node [anchor=north west][inner sep=0.75pt]    {$0$};
% Text Node
\draw (251,103.4) node [anchor=north west][inner sep=0.75pt]    {$\delta $};
% Text Node
\draw (601,103.4) node [anchor=north west][inner sep=0.75pt]    {$0$};
% Text Node
\draw (651,103.4) node [anchor=north west][inner sep=0.75pt]    {$0$};
% Text Node
\draw (551,103.4) node [anchor=north west][inner sep=0.75pt]    {$0$};
% Text Node
\draw (451,103.4) node [anchor=north west][inner sep=0.75pt]    {$0$};
% Text Node
\draw (113,243.4) node [anchor=north west][inner sep=0.75pt]    {$0$};
% Text Node
\draw (163,243.4) node [anchor=north west][inner sep=0.75pt]    {$0$};
% Text Node
\draw (463,243.4) node [anchor=north west][inner sep=0.75pt]    {$0$};
% Text Node
\draw (263,243.4) node [anchor=north west][inner sep=0.75pt]    {$\delta $};
% Text Node
\draw (363,243.4) node [anchor=north west][inner sep=0.75pt]    {$\delta $};
% Text Node
\draw (313,243.4) node [anchor=north west][inner sep=0.75pt]    {$\delta $};
% Text Node
\draw (212,243.4) node [anchor=north west][inner sep=0.75pt]    {$0$};
% Text Node
\draw (563,243.4) node [anchor=north west][inner sep=0.75pt]    {$0$};
% Text Node
\draw (613,243.4) node [anchor=north west][inner sep=0.75pt]    {$0$};
% Text Node
\draw (513,243.4) node [anchor=north west][inner sep=0.75pt]    {$0$};
% Text Node
\draw (413,243.4) node [anchor=north west][inner sep=0.75pt]    {$0$};
% Text Node
\draw (40,34.4) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$s_{j}$};
% Text Node
\draw (108,99.4) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$s'_{j}$};
\draw (64,246.4) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$v_{j}$};
\draw (198,276) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$j=r'$};
\draw (348,279) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$j=r_x$};
% Text Node
\draw (279,156.4) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$v_{j} ={\textstyle \sum _{k=0}^{j}} s_{k} -s'_{k}$};


\end{tikzpicture}
\end{tabular}
  \caption{One-Hot list to difference list}
  \label{fig:onehot}
 \end{figure}
\subsection{Look-up Table Based Verification}
\noindent Several works \cite{table0, table1, table2} employ look-up tables rather than boolean circuits for function evaluation. Notably, \cite{table0} proposes a semi-honest secure lookup table evaluation approach that relies solely on the output size communication cost during the online phase. This is achieved by utilizing the 2-PC replicated secret share protocol proposed by \cite{aby2} on $\mathbb{Z}_2$. %However, it is worth mentioning that \cite{table0} incurs a communication cost of $O(2^\lambda)$ during the setup phase, where $\lambda$ is the input size of the lookup table. 
In this work, we propose a novel maliciously secure look-up tables evaluation protocol. 

%Compared to \cite{table0}, our protocol has: 1)the same online phase performance and less communication overhead which is $O(\kappa \lambda)$ in the offline phase; 2) The ability to defend against a malicious adversary through the dual executions.

Specifically, we leverage the look-up table evaluation protocol to verify the correctness of non-linear function evaluation in the postprocessing phase. This approach efficiently allows us to verify whether $\mathcal{C}(r_x, m_x) = 1$ with the share value of $\langle x \rangle$. By utilizing the look-up table, we can efficiently validate the desired condition and ensure the correctness of the protocol evaluation. 
%Without loss of generality, consider verify a non-linear function $F(\langle x_1 \rangle, \ldots, \langle x_n \rangle) = c$, all parties can transfer it to verify $\mathcal{C}(r_{x_1}||\ldots||r_{x_n},m_{x_1}||\ldots||m_{x_n}||c) = 1$. 
Our technique can also apply batch-size verification, which cost $4\lambda + 6\lambda\kappa$ bits communication in the online phase for any $N$ pairs evaluation result need to verification. %At a high level, all parties perform a malicious security look-up table evaluation protocol to calculate $\mathcal{C}(r_x, m_x)$ and check if it is equal to $1$.  
%Our technique is start from that: $P_1$ and $P_2$ can locally generate the look-up table as Fig~.\ref{fig:table}(a), and locally evaluate the look-up table as Fig.~\ref{fig:table}(b). Due to the $r_x$ being generated in the setup phase, $P_0$ can secretly share the one-hot list $i \overset{?}{=} r_x$ at the same time. 

Our technique begins by allowing $P_1$ and $P_2$ to locally generate the look-up table, as shown in Fig.~\ref{fig:table}(a), where each item $\mathcal{C}(r, m_x)$ is assigned to look-up table $T(r)$. To evaluate look-up table as like Fig.~\ref{fig:table}(b), $P_0$ distribute the one-hot list $[s_j]$ in the setup phase such that $\{s_j := (j \overset{?}{=} r_x)\}_{j \in \ZZ_{2^\ell}}$.
Subsequently, $P_1,P_2$ can independently evaluate the look-up table, as illustrated in Fig.~\ref{fig:table}(b), to get the $[\cdot]$-share of $\mathcal{C}(r_x, m_x)$.
After that, $P_0, P_1$ can reveal $\mathcal{C}(r_x, m_x) $  to verify  $\mathcal{C}(r_x, m_x) = 1$.
%Since $r_x$ is generated during the setup phase, $P_0$ can simultaneously distribute the one-hot list $\{s_j := (j \overset{?}{=} r_x)\}_{j \in \ZZ_{2^\ell}}$ with DPF functionality $\{\mathcal{K}^{1, 1}_{r_x},\mathcal{K}^{1, 2}_{r_x}\}\leftarrow\Fgen^\ell(r_x, 1) $. 

The procedure of distributing the one-hot list requires the communication cost of $O(2^\ell)$.
In our communication friendly scheme(CF.~\ref{reduccomm}), we utilize  \cite{FSS}'s technique to reduce the overhead of sending one-hot list in the offline phase. 
 
  
The remained question is to achieve malicious security.
The misbehavior of ${P_1, P_2}$ and $P_0$ exhibits distinct characteristics. In the case of malicious $P_0$, who only participates in the offline phase, she can launch a selective failure attack by distributing the incorrect one-hot list, which lead to output $\mathcal{C}(r'_x, m_x)$ for adversary selected $r'_x$.  In the case of malicious  $P_1$ or $P_2$. The adversary can introduce an additive error  to manipulate the evaluation result. To  identify and prevent these misbehaviors, we employ a dual verification protocol.


\myhalfbox{ Protocol $\Pchk^\ell (\{[ x_i ]^{\ell}\}_{i \in |N|})$}{white!40}{white!10}{
    \footnotesize
    \emph{Input:} A list of $[\cdot]$-shared value. 
  
  \emph{Output:} $P_k$ output $x_i \overset{?}{=} 0$ for all $i \in |N|$.
  
    \underline{\textbf{Preprocessing:}}
    \begin{itemize}[leftmargin=*]
    \item[-] $P_1,P_2$ pick random value $m_x, \delta \leftarrow\ZZ_{2^\ell}$ together;
	\item[-] All parties invoke $\langle \alpha \rangle^{\ell[x]} \leftarrow \Pshc^{\ell[x]}$. 
	
	\end{itemize}

    \smallskip
    
    \underline{\textbf{Online:}}
    \begin{itemize}[leftmargin=*]
    \item[-]$P_j$ for $j \in \{1,2\}$ set $[x]^{\ell}:= \sum^{N}_{i = 1}\delta^i \cdot [x_i]^\ell$.
    \item[-]$P_j$ for $j \in \{1,2\}$ calculate $m_x - [x]^{\ell}$ and reveal to $P_0$.
    \item[-]$P_0$ sets $r_{x} = m_x - [x]^{\ell}$.
    \item[-]All parties perform:
    \begin{itemize}
    \item Local transfer $\langle x \rangle$ to $\langle x \rangle^{\ell[x]}$;
    \item Invoke $\Pple^{\ell[x]}$ to evaluate $\langle \Delta \rangle^{\ell[x]}= \langle \alpha \rangle^{\ell[x]} \cdot \langle x \rangle^{\ell[x]}$;
    \item Call $\Prec^{\ell[x]}(\langle \Delta \rangle^{\ell[x]}; P_1)$ and $\Prec^{\ell[x]}(\langle \Delta \rangle^{\ell[x]}; P_2)$.
    \end{itemize}
    \item[-] $P_j$ for $j \in \{1,2\}$ returns $1$ if $\Delta = 0$, otherwise return $0$.
    \end{itemize}
         \medskip
         }{ The Secure Zero Check Protocol   \label{fig:saf_rev}}
         
 \myhalfbox{ Protocol $\Pcps^{\ell} (\langle x \rangle^\ell, \mathcal{C} )$}{white!20}{white!10}{
    \footnotesize
  \emph{Input:} Verification circuit $\mathcal{C}$ with output $0/1$; $\langle \cdot \rangle^\ell$-shared value of $x$. 
  
  \emph{Output:} $\mathcal{C}(r_x, m_x) \overset{?}{=} 1$.
  
     \underline{\textbf{Preprocessing:}}
    \begin{itemize}[leftmargin=*]
    	\item[-] $P_0,P_1$ generate a random value $\delta_1 \in \ZZ_{2^\ell}$ together, and $P_0,P_2$ generate a random value $\delta_2 \in \ZZ_{2^\ell}$ together. $P_0$, $P_1$ generate $r' \in \ZZ_{2^\ell}$ together,
    	\item[-] $P_0$ prapares two one-hot list $\{s_j\}_{j \in |2^{\ell}|}$,$\{t_j\}_{j \in |2^{\ell}|}$ where $s_{r_x} = \delta_1$, $t_{r_x} = \delta_2$, and invoke $\Psha^\ell(s_j)$, $\Psha^\ell(t_j)$ for $j \in |2^{\ell}|$.
	 %pairs of DPF keys $\{\mathcal{K}^{\delta_1,1}_{r_x}, \mathcal{K}^{\delta_1,2}_{r_x}\}$, $\{\mathcal{K}^{\delta_2,1}_{r_x}, \mathcal{K}^{\delta_2,2}_{r_x}\}$. $P_0$ distributes DPF keys to other parties while $P_i$ for $i \in \{1,2\}$ hold $\mathcal{K}^{\delta_1,i}_{r_x},\mathcal{K}^{\delta_2,i}_{r_x}$.
	\item[-] $P_1$ generate another one-hot list $\{s'_j\}_{j \in |2^{\ell}|}$ where $s_{r'} = \delta_1$ and invoke $\Psha^\ell(s'_j)$ for $j \in |2^{\ell}|$.
	%prapares a pair of DPF keys $\mathcal{K}^{\delta_1,1}_{r'}$ and $\mathcal{K}^{\delta_1,2}_{r'}$, and sends $\mathcal{K}^{\delta_1,2}_{r'}$ to $P_2$.
	\item[-] $P_2$ generate another one-hot list $\{t'_j\}_{j \in |2^{\ell}|}$ where $t_{r'} = \delta_2$ and invoke $\Psha^\ell(t'_j)$ for $j \in |2^{\ell}|$.
	%prapares a pair of DPF keys $\mathcal{K}^{\delta_2,1}_{r'}$ and $\mathcal{K}^{\delta_2,2}_{r'}$, and sends $\mathcal{K}^{\delta_2,1}_{r'}$ to $P_1$.
	\item[-] $P_i$ for $i \in \{1,2\}$ calculate $\langle \Delta_1 \rangle^{\ell} = \langle \delta_1 \rangle^{\ell} \cdot(\langle r_x \rangle^{\ell}- r')$,$\langle \Delta_2 \rangle^{\ell} = \langle \delta_2 \rangle^{\ell}\cdot(\langle r_x \rangle^{\ell} - r')$ with $\Pmul$ (locally transfer $[\cdot]$ to $\langle \cdot \rangle$).
	\item[-] $P_i$ for $i \in \{1,2\}$ set $[\Delta_1]^\ell = m_x - [\Delta_1]^\ell$,$[\Delta_2]^\ell = m_x - [\Delta_2]^\ell$
	\end{itemize}

    \smallskip
    
    \underline{\textbf{Online:}}
	\begin{itemize}[leftmargin=*]
	\item[-] $P_i$, for $i \in \{1,2\}$ locally does:
	\begin{enumerate}
		\item generates a table $T$ while $T(j) = \mathcal{C}(j, m_x) \in \{0,1\}$ for all $j \in |2^{\ell}|$;
		\item calculates $[z_1]_i = \sum^{2^\ell}_{j=1}(T(j) \cdot [s_j])$,$[z_2]_i = \sum^{2^\ell}_{j=1}(T(j) \cdot [t_j])$;
		\item calculates $[u_1] =\sum^\ell_{k = 1}(\sum^k_{j = 1} [s_j] - \sum^k_{j = 1} [s'_j])$, $[u_2] = \sum^\ell_{k = 1}(\sum^k_{j = 1} [t_j] - \sum^k_{j = 1} [t'_j])$;
		\item reveal $[z_1]$ to $P_1$, $[z_2]$ to $P_2$.
	\end{enumerate}
	\item[-] All parties invoke $\Pchk(\{[u_i] - [\Delta_i]\}_{i \in |2|})$ and $P_i$ for $i \in \{1,2\}$ both get the output $\Delta'_i$.
	%$[\Delta'_1] = [u] - [\Delta_1]$, $[z_1]$ to $P_1$, $[\Delta'_2] = [v] - [\Delta_2]$, $[z_2]$ to $P_2$.
		\item[-] $P_i$ for $i \in \{1,2\}$ returns $1$ if $\Delta'_i = 1 \land z_i = \delta_i$ else $0$;
	\end{itemize}
        \smallskip
}{ The $P_1,P_2$-Dual Verified Protocol with Verificaiton Circuit $\mathcal{C}$.  \label{fig:CCP}}
\noindent \textbf{$P_1,P_2$-Dual Verified Protocol.} 
Specifically, to detect $P_1,P_2$'s misbehavior, $P_0$ can set the one-hot list value $\delta$($s_{r_x} = \delta$) instead of $1$ which is also secret for $P_1,P_2$ so that the malicious $P_1$ or $P_2$ can not flip the result to a legal result. In the case of $P_0$'s corruption, we introduce a differential check method, as shown in Fig.~\ref{fig:onehot}. One of $P_1,P_2$(e.g. $P_1$) can generate another pair of one-hot list $\{[s'_j]\}_{j \in \ZZ_{2^\ell}}$ while $s'_{r'} = \delta$. Then $P_1, P_2$ calculate the differential list $\{v_j\}_{j \in \ZZ_{2^\ell}}$ as Fig.~\ref{fig:onehot}.
 Subsequently, $P_1$ and $P_2$ reveal $\Delta = (\sum^{2^\ell}_j v_j) - \delta \cdot (r_x - r')$ to $P_1$ to check $\Delta = 0$.  We let $P_0$, $P_1$ calculate share of $\delta \cdot (r_x - r')$ in the preprocessing phase, with the malicious multiplication protocol. 
It is worth noting that $\delta$ is known to  $P_1$, which allows for potential manipulation of the result with an additive error.  To address this, our technique employs dual execution, ensuring that both $P_1$ and $P_2$ generate the verification one-hot list. Furthermore, directly leaking $\Delta$ to $P_1$ poses security risks since $P_1$ can potentially obtain the value of $r_x$ by distributing inconsistent $r'$ and one-hot list. To address this vulnerability, we apply a secure zero-checking protocol $\Pchk$(Fig.~\ref{fig:saf_rev}) to mitigate the risk.
 The detail of our dual verification protocol $\Pcps$ is illustrated in Fig.\ref{fig:CCP}. 
  \begin{lemma}
\label{zerochek}
To verify $x_i = 0$ for all $i \in |N|$, the protocol $\Pchk$ can ensure privacy if one of $P_1$ and $P_2$ is malicious and ensure the soundness if $P_0$ is malicious.
\end{lemma}
 \begin{proofsketch} 
 \textbf{Case I}: For malicious $P_0$, the only thing $P_0$ can do is to participate in the calculation of $\Delta$. Refer to  Lemma.~\ref{polyvv}, the soundness error is $2^{-\kappa}$.
 \textbf{Case II}: For malicious $P_1$, because $\alpha$ is uniform random and unknown to $P_1$, $P_1$ get no information about $x$.
 \end{proofsketch} 
\begin{lemma}
\label{cirvv}
The protocol $\Pcps$ securely verifies $\mathcal{C}(r_x, m_x) = 1$, in the presence of one malicious adversary.
\end{lemma}
\begin{proofsketch} 
  For malicious $P_0$, $P_0$ can generate wrong list $\{\hat{s}_j\}_{j \in |2^\ell|}$. Since $r'$ is uniform random and unknown to $P_0$, the probability that $P_0$ constructs a new list $\{\hat{s}_j\}_{j \in |2^\ell|}$ so that $[u_i] - [\Delta_i] = 0$ is $2^{-\ell}$.
  We discuss the situation of malicious $P_1$(Similar to $P_2$). \textbf{Soundness}: it is trivial to show that the probability $P_1$ set $[z_2]_1 = \sum^{2^\ell}_{j=1}(T(j) \cdot [t_j]) + e$  to make $[z_2]_1 + [z_2]_2 = \delta_1$ is $2^{-\ell}$, because  $\delta_1$ is unknown to $P_1$. \textbf{Privacy}: It is sufficient to show that $P_1$ learn nothing from $z_1$, due to the uniform random list $[s_j]_1$. Refer to Lemma.\ref{zerochek}, $P_1$ know nothing about $\Delta'_i$ except $\Delta'_i \overset{?}{=} 0$.
 \end{proofsketch} 

\noindent \textbf{Apply Batch Verification.}
Our protocol can obtain a constant online phase communication of batch verification. For the j-th execution of $\Pcps$ intermediate results $z^{(j)}_i$, $[u_i^{(j)}]$, $[\Delta_i^{(j)}]$,$\delta^{(j)}_i$, $P_i$ can verify the summerizing $\sum^N_{j = 1} ([ z^{(j)}_i] - \delta^{(j)}_i) = 1$ and invoke $\Pchk(\{[u_i]^{(j)} - [\Delta^{(j)}_i]\}_{i\in|2|,j \in |N|})$ with constant communication cost.
 %summerizing all $z_i$ in step 5 of Fig.~\ref{fig:CCP}. 2) Roughly speaking, for N pairs inputs need to be verified $\{\langle x^k \rangle\}_{k\in|N|}$,  $P_i$ can verify all intermediate outputs by calculating $\sum (\langle z_i^k \rangle - \delta^k_i) = 1$ and $\sum_k {\Delta'}^k_i = 0$. 
 We use $\Pcps^{\ell} (\{\langle x_i \rangle\}_{i \in |N|}, \mathcal{C} )$ to denote the batch verification protocol, which requires $1$ rounds and linear communication of $N\cdot(2^{\ell + 1}\ell + 6\ell)$ bits in the offline phase and requires $2$ rounds and constant communication of $4\ell + 6\ell\kappa$ bits in the online phase for $N$ pairs of multiplication triples.


%\myhalfbox{ Protocol $\Pcps^\ell (r_x, m_x, \mathcal{C} )$}{white!20}{white!10}{
%    \footnotesize
%  \emph{Input:} Common input verification circuit $\mathcal{C}$ with output $0/1$; $P_0$ inputs $r_x\in \ZZ_{2^{\ell}}$ in preprocessing phase, $P_1$,$P_2$ inputs $m_x \in \ZZ_{2^\gamma}$ ($\gamma$ can be any value) in online phase. 
%  
%  \emph{Output:} $P_0$ verify if $\mathcal{C}(r_x, m_x) = 1$.
%  
%     \underline{\textbf{Preprocessing:}}
%    \begin{itemize}[leftmargin=*]
%    	\item[-] $P_0$ prapares a pair of DPF keys $\mathcal{K}^{\Delta,1}_{r_x}$ and $\mathcal{K}^{\Delta,2}_{r_x}$. $P_0$ distributes DPF keys to other parties while $P_i$ for $i \in \{1,2\}$ hold $\mathcal{K}^{\Delta,i}_{r_x}$.
%	\end{itemize}
%
%    \smallskip
%    
%    \underline{\textbf{Online:}}
%	\begin{itemize}[leftmargin=*]
%	\item[-] $P_i$, for $i \in \{1,2\}$ generates a table $T$ while $T(j) = \mathcal{C}(j, m_x) \in \{0,1\}$ for all $j \in |2^{\ell}|$.
%	\item[-] $P_i$, for $i \in \{1,2\}$ calls $\mathcal{F}_\mathsf{expend}(\mathcal{K}^{\Delta,i}_{r_x})$ to get $\{s_j\}_{j \in |2^{\ell}|}$ and calculates $[z]_i = \sum^{2^\ell}_{j=1}(T(j) \cdot s_j)$.
%	\item[-] $P_i$, for $i \in \{1,2\}$ sends their shares to $P_0$ to reconstruct $z$.
%	\item[-] $P_0$ return $1$ if $z = \Delta$ else $0$.
%	\end{itemize}
%        \smallskip
%}{ The $P_0$ audit protocol with verificaiton circuit $\mathcal{C}$.  \label{fig:CCP}}   
%
%\myhalfbox{ Protocol $\Pcps^{\ell} (r_x, m_x, \mathcal{C} )$}{white!20}{white!10}{
%    \footnotesize
%  \emph{Input:} Common input verification circuit $\mathcal{C}$ with output $0/1$; $P_0$ inputs $r_x\in \ZZ_{2^{\ell}}$ in preprocessing phase, $P_1$,$P_2$ inputs $m_x \in \ZZ_{2^\gamma}$ ($\gamma$ can be any value) in online phase. 
%  
%  \emph{Output:} $P_1$ verify if $\mathcal{C}(r_x, m_x) = 1$.
%  
%     \underline{\textbf{Preprocessing:}}
%    \begin{itemize}[leftmargin=*]
%    	\item[-] $P_0$ prapares a pair of DPF keys $\mathcal{K}^{1,1}_{r_x}$ and $\mathcal{K}^{1,2}_{r_x}$. $P_0$ distributes DPF keys to other parties while $P_i$ for $i \in \{1,2\}$ hold $\mathcal{K}^{1,i}_{r_x}$.
%	\item[-] $P_2$ prapares a pair of DPF keys $\mathcal{K}^{1,1}_{r'}$ and $\mathcal{K}^{1,2}_{r'}$, and sends $\mathcal{K}^{1,2}_{r'}$ to $P_1$.
%	\item[-] $P_i$ for $i \in \{1,2\}$ calculate $[\Delta] = [r_x] - r'$ and reveal it to $P_1$.
%	\end{itemize}
%
%    \smallskip
%    
%    \underline{\textbf{Online:}}
%	\begin{itemize}[leftmargin=*]
%	\item[-] $P_i$, for $i \in \{1,2\}$ locally does:
%	\begin{itemize}
%		\item generates a table $T$ while $T(j) = \mathcal{C}(j, m_x) \in \{0,1\}$ for all $j \in |2^{\ell}|$;
%		\item calls $\mathcal{F}_\mathsf{expend}(\mathcal{K}^{1,i}_{r_x})$ to get $\{[s_j]\}_{j \in |2^{\ell}|}$ and calculates $[z]_i = \sum^{2^\ell}_{j=1}(T(j) \cdot [s_j])$;
%		%\item calls $\mathcal{F}_\mathsf{expend}(\mathcal{K}^{1,i}_{r'})$ to get $\{[s'_j]\}_{j \in |2^{\ell}|}$;
%		\item calls $\mathcal{F}_\mathsf{expend}(\mathcal{K}^{\delta,i}_{r_x})$ to get $\{[t_j]\}_{j \in |2^{\ell}|}$;
%		\item calculates $[u_j] = \sum_k [s_j]$, $[u'_j] = \sum_k [s'_j]$, $[v] = \sum_j ([s_j] - [s'_j])$;
%		%\item $\sum_k [t_j] + [s_j]$
%	\end{itemize}
%	\item[-] $P_2$ send $[v]_2$,$[z]_2$ to $P_1$ and $P_1$ returns $1$ if $v = \Delta \land z = 1$ else $0$;
%	
%	\end{itemize}
%        \smallskip
%}{ The $P_1$ audit protocol with verificaiton circuit $\mathcal{C}$.  \label{fig:CCP}}   



==> subject/related.tex <==
%!TEX root = ../main.tex

\section{Related work}
%In honest-majority setting, an array of works \cite{YAS, KDK, TurboPack, FastRing, Yet, ATLAS} design protocols for efficient secure multi-party computation. Compared with the semi-honest case, previous work requires many times the additional overhead to defend against malicious threat adversaries under the honest majority. \cite{YAS} has designed two sets of schemes, which requires the communication overhead of $42\cdot n$ or $5(n^2-n)$ ring elements of each multiplication, for $n$ parties. \cite{KDK} reduce the communication to $42\cdot n$. For 3-party computation, \cite{KDK} only need $2$ ring elements. \cite{ATLAS} further r\elleduces the communication overhead by introducing batch verification and a series of other optimization techniques. \cite{ATLAS}'s protocols require a two-round communication overhead of $2n$ field element or a one-round communication overhead of $3n$ field element, however, \cite{ATLAS}'s protocol can only run on the field. \cite{TurboPack} achieves a constant online phase communication overhead ($12$ field elements) with the help of packed secret sharing technology, but the cost is that it requires a total of $10n+44$ field elements communication overhead for each multiplication. The work of  \cite{FastRing} refocuses on the MPC in ring, it achieves $1 \frac{1}{3}$ ring elements with two rounds communication or $1 \frac{2}{3}$ ring elements with one round communication.
\noindent
In the honest-majority setting, several works such as \cite{YAS, KDK, TurboPack, FastRing, Yet, ATLAS} have designed protocols for efficient secure multi-party computation against the malicious adversary. However, compared to the semi-honest case, previous work requires significantly higher additional overhead, while \cite{YAS} requires $42 \cdot n$ or $5(n^2-n)$ ring elements for each multiplication ($n$ represents the number of parties); \cite{ATLAS} requires $2n$ field elements; \cite{TurboPack} achieves a constant online phase communication overhead of $12$ field elements; %However, this comes at the cost of a total communication overhead of $10n+44$ field elements for each multiplication. 
\cite{FastRing} achieves a communication overhead of $1 \frac{1}{3}$ ring elements with two rounds of communication or $1 \frac{2}{3}$ ring elements with one round of communication.
With the advancement of the maliciously secure multiplication protocol, practical maliciously secure privacy-preserving machine learning becomes attainable. 
\cite{SecureML,ASTRA,aby3, ASTRA, FALCON, Trident, FLASH, BLAZE, swift} realize privacy-preserving machine learning protocols under the malicious threat model in an honest majority.
In the semi-honest setting, protocols such as \cite{aby3, ASTRA, aby2, BLAZE} are all based on three parties replicated secret sharing, which only request $3$ ring elements communication each multiplication. The online phase communication overhead of $2$ ring elements can be achieved by handing over part of the communication to a circuit-dependent offline phase \cite{ASTRA}.
In the malicious setting, a series of optimizations \cite{ASTRA, BLAZE, swift} reduced the multiplication overhead to 6 ring elements ($3$ in the offline phase) in the three-party setting. To evaluate non-linear functions such as ReLU and Maxpool, protocols like \cite{aby3, swift, aby2} employ a conversion process that transforms arithmetic secret sharing into boolean secret sharing. Subsequently, they utilize this boolean secret-sharing scheme to evaluate corresponding non-linear functions. The disadvantage of this approach is the need to introduce $\log \ell$ rounds of communication. 
Furthermore, in protocols such as \cite{aby3, BLAZE, ASTRA}, garbled circuits are employed for evaluating non-linear functions. The use of garbled circuits introduces a significant amount of additional communication overhead, particularly in the presence of a malicious threat model.
In contrast, the protocols described in \cite{SecureNN, CrypTFlow} tackle the sign-bit extraction problem with a constant round communication overhead, while they require a substantial communication overhead of $10$ rounds, which can be even larger than $\log\ell$ rounds when $\ell$ is small.
On the other hand, \cite{Bicoptor} implements comparison through a truncation protocol. Their approach performs local truncation $\ell$ times, followed by involving a third party to verify if the result contains zero items. This scheme realizes two rounds of $\ell^2$ bits communication. However, this approach has not been applied to malicious threat models.


==> subject/security.tex <==
%!TEX root = ../main.tex
\section{Security Model}
We analyze the security of our protocols in the well-known Universal Composibility (UC) framework~\cite{UC}, which follows the simulation-based security paradigm. 
 The adversary $\AAA$ is allowed to partially control the communication tapes of all uncorrupted machines, that is, it sees all the messages sent from and to the uncorrupted machines and controls the sequence in which they are delivered. Then, a protocol $\Pi$ is a secure realization of the functionality $\FFF$, if it satisfies that for every PPT adversary $\AAA$ attacking an execution of $\Pi$, there is another PPT adversary $\SSS$ (simulator) attacking the ideal process that uses $\FFF$ where the executions of $\Pi$ with $\AAA$ and that of $\FFF$ with $\SSS$ makes no difference to any PPT environment $\mathcal{Z}$.

 \emph{\underline{The idea world execution.}}  In the ideal world, the parties $\mathcal{P}:=\{P_0,P_1,P_2\}$ only communicate with the ideal functionality $\FFF_{3\mathsf{pc}}$ with the excuted function $f$. All parties send their share to $\FFF_{3\mathsf{pc}}$, $\FFF_{3\mathsf{pc}}$ calculate and output the result depend on the adversary $\SSS$. 
 
\myherebox{ Functionality $\FFF_{3\mathsf{pc}}$}{white!20}{white!10}{
  $\FFF_{3\mathsf{pc}}$ interacts with the parties in $\mathcal{P}$ and the adversary $\SSS$. Let $f$ denote the functionality to be computed.
  
  \underline{\textbf{Input:}}
  \begin{itemize}[leftmargin=*]
  \item Upon receiving from $(\mathsf{Input},\sid,x_i)$ from  $P_i\in \mathcal{P}$, record $x_i$ and send $(\mathsf{Input},\sid,P_i)$ to $\SSS$. 
    \end{itemize}
    
     \underline{\textbf{Execution:}}
  \begin{itemize}[leftmargin=*]
   \item Upon receiving $(\mathsf{Compute},\sid)$ from $\SSS$, if all $x_i$ are recorded  compute $( y_0,  y_1,  y_2) = f( x_0,  x_1,  x_2)$.
   \item For $i\in[3]$, send $(\mathsf{Output},  y_i)$ to $P_i$ via \emph{private delayed channel}. 
    \end{itemize} 
    


}{ The ideal functionality  $\FFF_{3\mathsf{pc}}$. \label{fig:Fmpc}} 


 
  \emph{\underline{The real world execution.}}  In the real world, the parties $\mathcal{P}:=\{P_0,P_1,P_2\}$ communicate with each other via secure channel functionality $\mathcal{F}_{\mathsf{sc}}$ for the protocol execution $\Pi$.  Our protocols work in the pre-processing model, but, for simplicity, we analyze the offline and online protocols together as a whole. 

\begin{definition}
We say protocol $\Pi$ UC-secure realizes functionality $\FFF$ if for all PPT adversaries $\AAA$ there exists a PPT simulator $\SSS$ such that for all PPT environment $\mathcal{Z}$ it holds:
$$
\mathsf{Real_{\Pi,\AAA,\mathcal{Z}}}(1^\lambda) \; \approx \;  \mathsf{Ideal_{\FFF,\SSS,\mathcal{Z}}}(1^\lambda) 
$$ 
\end{definition}
